Representation Learning of Tangled Key-Value Sequence Data for Early Classification

Key-value sequence data has become ubiquitous and naturally appears in a variety of real-world applications, ranging from the user-product purchasing sequences in e-commerce, to network packet sequences forwarded by routers in networking. Classifying these key-value sequences is important in many scenarios such as user profiling and malicious applications identification. In many time-sensitive scenarios, besides the requirement of classifying a key-value sequence accurately, it is also desired to classify a key-value sequence early, in order to respond fast. However, these two goals are conflicting in nature, and it is challenging to achieve them simultaneously. In this work, we formulate a novel tangled key-value sequence early classification problem, where a tangled key-value sequence is a mixture of several concurrent key-value sequences with different keys. The goal is to classify each individual key-value sequence sharing a same key both accurately and early. To address this problem, we propose a novel method, i.e., Key-Value sequence Early Co-classification (KVEC), which leverages both inner- and inter-correlations of items in a tangled key-value sequence through key correlation and value correlation to learn a better sequence representation. Meanwhile, a time-aware halting policy decides when to stop the ongoing key-value sequence and classify it based on current sequence representation. Experiments on both real-world and synthetic datasets demonstrate that our method outperforms the state-of-the-art baselines significantly. KVEC improves the prediction accuracy by up to $4.7 - 17.5\%$ under the same prediction earliness condition, and improves the harmonic mean of accuracy and earliness by up to $3.7 - 14.0\%$.

==> ss_exp_att_dist.tex <==




==> ss_inference.tex <==

\subsection{Streaming Inference}
In model optimization phase, parallelized attention computing accelerate training. However in proposed TKVSEC problem, for incoming sequence data, the no-streaning structure repeats redundant floating-point operations during the inference phase. For example, in ~\cref{Fig.no_stream_infer}, When the timestamp is 4, the model collects all data points before this moment as input, and calculates the latent vector at each position (the green block in the figure), and then when the timestamp moving to 5, the model recalculates the latent vector to get the current representation of the key-value sequence even though partial latent vectors have been computed at the previous moment.
\begin{figure}[!htb]
    \centering
    \subfloat[No-Streaming Inference\label{Fig.no_stream_infer}]{\includegraphics[width=1.0\linewidth]{no_streaming}}\\
    \subfloat[Streaming Inference\label{Fig.stream_infer}]{\includegraphics[width=1.0\linewidth]{streaming}}
    \caption{Streaming Inference}
    \label{fig:inference_phase}
\end{figure}

Inspired by, we propose real-time streaming inference framework such as ~\cref{Fig.stream_infer}, it change the parallel attention to serial computation and use external memory to cache the previous hidden vectors (the yellow block in the figure). At each timestamp, we only operate the imput embedding of the current item, and compute the dynamic relation self-attention score with the cached previous latent vectors, then appending the current latent vector to memory. For a key-value sequence length $T$ and halting in $\tau$

==> tab_symbols.tex <==
\begin{table}[htbp]
  \centering
  \caption{Frequently used symbols \label{tab:symbol}}
  \begin{tabular}{c|l}
    \hline
    \hline
    \textbf{Symbol}                            & \textbf{Description}                                  \\
    \hline
    $\CS$                                      & a tangled key-value sequence                          \\
    $\CS_k\subseteq\CS$                        & a key-value sequence sharing key $k$         \\
    $e=\pr{k,\bv}\in\CS$                       & an item with key $k$ and value $\bv$ \\
    $\bs_k^{(t)}$                               & representation vector of $\CS_k$ at time step $t$     \\
    $\bM^{(t)}$                                 & dynamic mask matrix                                   \\
    $\bE_0^{(t)},\bE_\mathrm{att}^{(t)},\bE^{(t)}$ & embedding matrices at time step $t$                   \\
    $y_k, \hat{y_k}$                            & ground truth label and the predicted label of $\CS_k$ \\
    $n_k$                                       & the least number of items collected from $\CS_k$ \\
    $K$                                       & the number of key-value sequences $\CS_k$ in $\CS$ \\
    \hline
  \end{tabular}
\end{table}

